dSphobic Dark Matter

We present a mechanism that allows thermal relic dark matter to annihilate efficiently in the Galactic Halo and in galaxy clusters, but not in the lower-velocity environments of dwarf spheroidal (dSph) galaxies. We realize this within a complete model in which the dark matter consists of two distinct states separated by a small mass splitting. An indirect detection signal is generated only through the coannihilations of these two states, requiring both to be present. In the halo of the Milky Way, the dark matter particles in the lighter state can be excited into the long-lived heavier state through scattering. Once excited, these heavier particles can coannihilate with those in the lighter state, yielding a gamma-ray signal with little or no suppression. By contrast, the dark matter particles in dwarf galaxies do not possess enough kinetic energy to be excited, thereby suppressing the coannihilation rate and corresponding indirect detection signals from those systems. This framework breaks the predictive relationship that ordinarily exists between these respective gamma-ray signals and complicates our ability to interpret the results of indirect detection searches.

==> packages_v2.tex <==
\usepackage{amsmath,amssymb,amsthm}
\usepackage{graphicx}
\usepackage[usenames, dvipsnames]{xcolor}
%\usepackage{hyperref}
%\usepackage{cite}
\usepackage{slashed}
%\usepackage{subfig}
\usepackage{tabularx}
\usepackage{empheq}
\usepackage{mathrsfs}
\usepackage{comment}
%\usepackage{hepunits}%commented out in December 2024
\usepackage{bbold}
\usepackage[shortlabels]{enumitem}

\usepackage{url}
\usepackage{color}

\definecolor{light-gray}{gray}{0.9}
\definecolor{medium-gray}{gray}{0.7}
\definecolor{darkblue}{rgb}{0.0,0.0,0.6}
\definecolor{red}{rgb}{0.9, 0,0}
\definecolor{navy}{rgb}{0.05, 0.05,0.8}
%\definecolor{linkcolor}{rgb}{0.65, 0.48, 0.36}
%\definecolor{linkcolor}{rgb}{0.0,0.5,0.4}
%\definecolor{linkcolor}{rgb}{0,0.5,0.8}
\definecolor{linkcolor}{rgb}{0.0, 0.28, 0.67}
\definecolor{paleblue}{rgb}{0.69, 0.93, 0.93}  

\usepackage[colorlinks]{hyperref}
\hypersetup{
     colorlinks   = true,
     citecolor    = linkcolor,
     linkcolor    = linkcolor,
     urlcolor    = linkcolor
     %citecolor    = MidnightBlue,
     %linkcolor    = MidnightBlue,
     %urlcolor    = MidnightBlue
}
